Vortex and Meissner phases of strongly-interacting bosons on a two-leg ladder

We establish the phase diagram of the strongly-interacting Bose-Hubbard model defined on a two-leg ladder geometry in the presence of a homogeneous flux. Our work is motivated by a recent experiment [Atala et al., Nature Phys. 10, 588 (2014)], which studied the same system, in the complementary regime of weak interactions. Based on extensive density matrix renormalization group simulations and a bosonization analysis, we fully explore the parameter space spanned by filling, inter-leg tunneling, and flux. As a main result, we demonstrate the existence of gapless and gapped Meissner and vortex phases, with the gapped states emerging in Mott-insulating regimes. We calculate experimentally accessible observables such as chiral currents and vortex patterns.

==> fig_entropy_MI_obc_pap.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  % Encoding inside the plot.  In the header of your document, this encoding
  % should to defined, e.g., by using
  % \usepackage[latin1,<other encodings>]{inputenc}
  \inputencoding{latin1}%
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(11338.00,3400.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(365,340){\makebox(0,0)[r]{\strut{} 0}}%
      \put(365,2861){\makebox(0,0)[r]{\strut{} 0.5}}%
      \put(425,190){\makebox(0,0){\strut{} 0}}%
      \put(2990,190){\makebox(0,0){\strut{} 0.5}}%
      \put(5555,190){\makebox(0,0){\strut{} 1}}%
      \put(85,1852){\rotatebox{-270}{\makebox(0,0){\strut{}\relsize{2.5}{$\SvN$}}}}%
      \put(4190,80){\makebox(0,0){\strut{}\relsize{2.5}{$\LA/L$}}}%
      \put(553,3063){\makebox(0,0)[l]{\strut{}\relsize{1.5}{(a)}}}%
      \put(2990,3063){\makebox(0,0){\strut{}\relsize{1.2}{$\boldsymbol{\phi=\pi/2}$, $\boldsymbol{n=0.5}$}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(5782,190){\makebox(0,0){\strut{} 0}}%
      \put(8347,190){\makebox(0,0){\strut{} 0.5}}%
      \put(10911,190){\makebox(0,0){\strut{} 1}}%
      \put(10911,340){\makebox(0,0)[l]{\strut{} 0}}%
      \put(10911,2357){\makebox(0,0)[l]{\strut{} 1}}%
      \put(11130,1852){\rotatebox{-270}{\makebox(0,0){\strut{}\relsize{2.5}{$\SvN$}}}}%
      \put(9546,80){\makebox(0,0){\strut{}\relsize{2.5}{$\LA/L$}}}%
      \put(5910,3063){\makebox(0,0)[l]{\strut{}\relsize{1.5}{(b)}}}%
      \put(8347,2760){\makebox(0,0){\strut{}\relsize{1.2}{$\boldsymbol{\phi=0.9\pi}$, $\boldsymbol{n=0.5}$}}}%
      \put(9372,945){\makebox(0,0){\strut{}fitting parameters:}}%
      \put(9372,718){\makebox(0,0){\strut{}$c=$ 1.037}}%
      \put(9372,491){\makebox(0,0){\strut{}$g=$ 0.659}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(7130,845){\makebox(0,0)[l]{\strut{}\relsize{1.2}{data}}}%
      \csname LTb\endcsname%
      \put(7130,645){\makebox(0,0)[l]{\strut{}\relsize{1.2}{fit}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{fig_entropy_MI_obc_pap}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> fig_gap_pap.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  % Encoding inside the plot.  In the header of your document, this encoding
  % should to defined, e.g., by using
  % \usepackage[latin1,<other encodings>]{inputenc}
  \inputencoding{latin1}%
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(11338.00,3400.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(506,340){\makebox(0,0)[r]{\strut{} 0}}%
      \put(506,1550){\makebox(0,0)[r]{\strut{} 1}}%
      \put(506,2760){\makebox(0,0)[r]{\strut{} 2}}%
      \put(566,190){\makebox(0,0){\strut{} 0}}%
      \put(2229,190){\makebox(0,0){\strut{} 1}}%
      \put(3892,190){\makebox(0,0){\strut{} 2}}%
      \put(5555,190){\makebox(0,0){\strut{} 3}}%
      \put(226,2152){\rotatebox{-270}{\makebox(0,0){\strut{}\relsize{2.5}{$\gapM/J$}}}}%
      \put(3060,80){\makebox(0,0){\strut{}\relsize{2.5}{$\Jperp/J$}}}%
      \put(815,3063){\makebox(0,0)[l]{\strut{}\relsize{1.5}{(a)}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1122,1909){\makebox(0,0)[l]{\strut{}\relsize{1.2}{fit by $\Jperp+\textrm{cst}$}}}%
      \csname LTb\endcsname%
      \put(1122,2109){\makebox(0,0)[l]{\strut{}\relsize{1.2}{$\phi/\pi=0.8$}}}%
      \csname LTb\endcsname%
      \put(1122,2309){\makebox(0,0)[l]{\strut{}\relsize{1.2}{$\phi/\pi=0.5$}}}%
      \csname LTb\endcsname%
      \put(1122,2509){\makebox(0,0)[l]{\strut{}\relsize{1.2}{$\phi/\pi=0.2$}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(5782,190){\makebox(0,0){\strut{} 0}}%
      \put(7445,190){\makebox(0,0){\strut{} 1}}%
      \put(9107,190){\makebox(0,0){\strut{} 2}}%
      \put(10770,190){\makebox(0,0){\strut{} 3}}%
      \put(10770,340){\makebox(0,0)[l]{\strut{} 0}}%
      \put(10770,1285){\makebox(0,0)[l]{\strut{} 1}}%
      \put(10770,2231){\makebox(0,0)[l]{\strut{} 2}}%
      \put(10770,3176){\makebox(0,0)[l]{\strut{} 3}}%
      \put(11169,1752){\rotatebox{-270}{\makebox(0,0){\strut{}\relsize{2.5}{$\gapEx/J$}}}}%
      \put(8276,80){\makebox(0,0){\strut{}\relsize{2.5}{$\Jperp/J$}}}%
      \put(6031,3063){\makebox(0,0)[l]{\strut{}\relsize{1.5}{(b)}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(6217,1909){\makebox(0,0)[l]{\strut{}\relsize{1.2}{fit by $2\Jperp+\textrm{cst}$}}}%
      \csname LTb\endcsname%
      \put(6217,2109){\makebox(0,0)[l]{\strut{}\relsize{1.2}{$\phi/\pi=0.8$}}}%
      \csname LTb\endcsname%
      \put(6217,2309){\makebox(0,0)[l]{\strut{}\relsize{1.2}{$\phi/\pi=0.5$}}}%
      \csname LTb\endcsname%
      \put(6217,2509){\makebox(0,0)[l]{\strut{}\relsize{1.2}{$\phi/\pi=0.2$}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{fig_gap_pap}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> fig_gap_pap2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  % Encoding inside the plot.  In the header of your document, this encoding
  % should to defined, e.g., by using
  % \usepackage[latin1,<other encodings>]{inputenc}
  \inputencoding{latin1}%
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(11338.00,3400.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(506,340){\makebox(0,0)[r]{\strut{} 0}}%
      \put(506,1550){\makebox(0,0)[r]{\strut{} 1}}%
      \put(506,2760){\makebox(0,0)[r]{\strut{} 2}}%
      \put(566,190){\makebox(0,0){\strut{} 0}}%
      \put(1813,190){\makebox(0,0){\strut{} 0.25}}%
      \put(3061,190){\makebox(0,0){\strut{} 0.5}}%
      \put(4308,190){\makebox(0,0){\strut{} 0.75}}%
      \put(5555,190){\makebox(0,0){\strut{} 1}}%
      \put(226,2152){\rotatebox{-270}{\makebox(0,0){\strut{}\relsize{2.5}{$\gapM/J$}}}}%
      \put(3780,80){\makebox(0,0){\strut{}\relsize{2.5}{$\phi/\pi$}}}%
      \put(815,3063){\makebox(0,0)[l]{\strut{}\relsize{1.5}{(a)}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1343,2811){\makebox(0,0)[l]{\strut{}\relsize{1.2}{$\Jperp/J=1$}}}%
      \csname LTb\endcsname%
      \put(1343,2611){\makebox(0,0)[l]{\strut{}\relsize{1.2}{$\Jperp/J=2$}}}%
      \csname LTb\endcsname%
      \put(1343,2411){\makebox(0,0)[l]{\strut{}\relsize{1.2}{$\Jperp/J=3$}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(5782,190){\makebox(0,0){\strut{} 0}}%
      \put(7029,190){\makebox(0,0){\strut{} 0.25}}%
      \put(8276,190){\makebox(0,0){\strut{} 0.5}}%
      \put(9523,190){\makebox(0,0){\strut{} 0.75}}%
      \put(10770,190){\makebox(0,0){\strut{} 1}}%
      \put(10770,340){\makebox(0,0)[l]{\strut{} 0}}%
      \put(10770,1853){\makebox(0,0)[l]{\strut{} 1}}%
      \put(10770,3365){\makebox(0,0)[l]{\strut{} 2}}%
      \put(11169,1752){\rotatebox{-270}{\makebox(0,0){\strut{}\relsize{2.5}{$\gapEx/J$}}}}%
      \put(8996,80){\makebox(0,0){\strut{}\relsize{2.5}{$\phi/\pi$}}}%
      \put(6031,3063){\makebox(0,0)[l]{\strut{}\relsize{1.5}{(b)}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(6558,2206){\makebox(0,0)[l]{\strut{}\relsize{1.2}{$\Jperp/J=1$}}}%
      \csname LTb\endcsname%
      \put(6558,2006){\makebox(0,0)[l]{\strut{}\relsize{1.2}{$\Jperp/J=2$}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{fig_gap_pap2}}%
    \gplfronttext
  \end{picture}%
\endgroup

